Hacking the Fabric: Targeting Partial Reconfiguration for Fault Injection in FPGA Fabrics

FPGAs are now ubiquitous in cloud computing infrastructures and reconfigurable system-on-chip, particularly for AI acceleration. Major cloud service providers such as Amazon and Microsoft are increasingly incorporating FPGAs for specialized compute-intensive tasks within their data centers. The availability of FPGAs in cloud data centers has opened up new opportunities for users to improve application performance by implementing customizable hardware accelerators directly on the FPGA fabric. However, the virtualization and sharing of FPGA resources among multiple users open up new security risks and threats. We present a novel fault attack methodology capable of causing persistent fault injections in partial bitstreams during the process of FPGA reconfiguration. This attack leverages power-wasters and is timed to inject faults into bitstreams as they are being loaded onto the FPGA through the reconfiguration manager, without needing to remain active throughout the entire reconfiguration process. Our experiments, conducted on a Pynq FPGA setup, demonstrate the feasibility of this attack on various partial application bitstreams, such as a neural network accelerator unit and a signal processing accelerator unit.

==> Countermeasures.tex <==
\section{Fault-Attack Detection Technique}
\subsection{Hash-based Authentication of Partial Bitstreams}
Error detection codes (EDCs) are widely used as countermeasures for detecting fault attacks. EDCs incur low hardware area overhead in their implementation. For example, parity check-based EDC technique has been employed in \cite{bertoni2004efficient}
to detect a byte fault attack in AES.

In this section, we explore an authentication mechanism, namely ASCON, to verify the integrity of a partial bitstream before it is configured on the FPGA. ASCON is a well-known family of hashing algorithms that has been standardized recently in the NIST Lightweight Cryptography competition and is part of the CAESAR competition for authenticated encryption \cite{dobraunig2021ascon}. We specifically use ASCON hashing to detect fault attacks in partial bitstreams because: 
\begin{itemize}[leftmargin=*,topsep=0pt]
    \item ASCON is lightweight and can be easily implemented within a reconfiguration manager.
    \item The hash is checked before the partial bitstream is loaded to the FPGA. Any alteration in the bitstream due to a fault attack will result in a different hash value than the expected hash. Therefore, if a persistent fault attack occurs during reconfiguration of the bitstream on the FPGA, the attack is detected and the bitstream is blocked from FPGA configuration.
    \item Many users typically disable CRC before configuring their partial bitstreams on the FPGA; CRC often generates an incorrect value that does not match the golden value, thus blocking the bitstream from being loaded to the FPGA \cite{6461919}. However, as noted in Section V.B, disabling the CRC allows the partial bitstreams to be configured to the FPGA even after fault injection, leading to erroneous computations. Hence, to preserve the integrity and security of the multi-tenant FPGA irrespective of the enabling/disabling of CRC, we integrate the ASCON framework within the reconfiguration manager. Therefore, even with CRC disabled, any fault introduced into the partial bitstream is detected, ensuring that only authenticated bitstreams are loaded to the FPGA.
\end{itemize}  

\begin{figure}
\centering
\includegraphics[width=0.47\textwidth]{Figures/ascon.pdf}

\caption{Implementation of ASCON in CoRQ framework for detecting fault attack on partial bitstreams.}
\label{defense}
\vspace{-0.4cm}
\end{figure}

We implement the ASCON authentication technique within CoRQ. The proposed fault-detection framework is shown in Fig. \ref{defense}. ASCON performs authenticated encryption of 128 bits at a time. A group of 128 bits is known as a block. Therefore, an input bitstream of length $k$ bits can be converted into $m$ blocks, where $m=\frac{k}{128}$. The value of $m$ is dependent on the specific bitstream to be authenticated. For our experiments, we use three bitstreams, namely blinkline, blinkcount, and blinkall. We  pre-compute the golden hash values using ASCON corresponding to each evaluated bitstream, and hardcode these values as a constant in the VHDL implementation of CoRQ memory. The pseudocode of ASCON hash-based authentication is described in Fig. \ref{pseudocode}. 

We next prove some important security properties of ASCON when it is used to detect fault attacks on CoRQ.

\textbf{Lemma 1:} If $T$ and $T'$ are two  bitstreams such that $T\neq T'$, then $H(T)\neq H(T')$, where $H(T)$ and $H(T')$ are the computed hash values using ASCON.

\textit{Proof:}
As a  hash-based authentication scheme, ASCON is \textit{collision-resistant} \cite{dobraunig2021ascon}. This means that it is computationally impossible to find two distinct bitstreams $T$ and $T'$ such that $H(T)=H(T')$. When a bitstream $T$ is preloaded into CoRQ, it is authenticated using ASCON. If a fault attack changes the bitstream to $T'$, the resulting hash $H(T')$ will differ significantly from $H(T)$, because of the intermediate computations shown in Fig. \ref{pseudocode}. If $H(T')$ does not match the golden reference $H(T)$, it indicates that a fault attack has occurred and the fault-injected bitstream is blocked from dynamic reconfiguration on the FPGA.\hfill$\Box$

\textbf{Lemma 2:} Using ASCON, the exact block(s) impacted by a fault attack can be identified.

\textit{Proof:} As depicted in Fig. \ref{pseudocode}, ASCON processes a bitstream in a block-wise manner, where the hash value computed for each block is dependent on the hash value of the preceding block. For enhanced fault-detection granularity, we can insert $x$ number of checkpoints in Fig. \ref{pseudocode}, where $2\leq x\leq m$. By storing multiple checkpoints, it is possible to maintain multiple golden hash values instead of storing only one golden hash value for a particular bitstream. This allows a precise detection and localization of fault-induced manipulations within the bitstream. If a fault is induced in a particular block, the hash value corresponding to that block will differ from the golden value, thereby identifying the exact block(s) affected.  \hfill$\Box$

We implemented ASCON within  CoRQ on the Pynq-Z1 FPGA and evaluated the FPGA resource usage in Table \ref{overhead}. We observe that the fault-detection scheme incurs a low resource utilization in terms of the number of LUTs and registers, therefore the overhead for fault-attack detection is low.
\textcolor{blue}{ASCON detects the persistent fault attack when the bitstream is preloaded to CoRQ, and prevents the faulty bitstream from being dynamically reconfigured on the FPGA. Note that when a fault attack is detected, only that specific faulty bitstream is prevented from being reconfigured; the remaining bitstreams which are not faulty can still be loaded to the FPGA. This is in contrast to CRC, which blocks fault-free bitstreams from loading to the FPGA when a faulty bitstream is detected.}

\begin{figure}
\begin{algorithm}[H]
\fontsize{7}{0}{
\SetAlgoLined
\footnotesize\\
    \KwInput{ \fontsize{8}{8}{}User input bitstream $T$}
\KwOutput {Detects a fault-injected bitstream $flt\_status$} 
    \textbf{Algorithm:}{$ASCON$}
    \\
    
   $block[m]$$\gets$ Split $T$ into $m$ blocks /*ASCON performs authenticated encryption of 1 block at a time*/ \\

    $H_{block[0]}\gets ASCON(block[0]) $  \\
    \For{$i$ in range($1, m$)}{
    $H_{block[i]}\gets ASCON(block[i])\oplus H_{block[i]} )$
    }
    
    
 \If{$H_{block[m-1]}==H^*$ } {
  $flt\_status\gets false$} \\
  \Else{$flt\_status\gets true$}}
  
 
   

     
   
   \Return $flt\_status$ \\
       

\end{algorithm}

\caption{Pseudocode for detecting a fault attack on a partial bitstream using ASCON-based authentication.}\label{pseudocode}


% \end{algorithm} 
% \vspace{-0.2cm}

\end{figure}

% ASCON performs authenticated encryption using 64-bit blocks, processing one block at a time

% Alternatively, we can pass the golden reference as an argument to the CoRQ.

% bitstreams has 32-bit words. ASCON works on every 128 bits. 1 block is 128 bits. calculates 

% 4n words
% 4n = m blocks
% hash block0 = ascon(block0)
% for i = 1 to m
% hash blocki = ascon(blocki) xor hash block(i-1)

% check hash(m-1) = golden reference


 


\begin{table}
\centering
\caption{The number of LUTs and registers used by the hash-based authentication scheme on the Pynq-Z1 FPGA.}
%\fontsize{8.2}{8.2}\selectfont
\small
\begin{tabular}{|c |c |c|c|c|} 
\cline{1-5}
Design&{\# LUTs}& \# Registers&\%LUT&\%Registers \\
\hline
CoRQ&4030&3060&7.5&2.8 \\
CoRQ+ASCON&5567&3729&10.46&3.5 \\



\hline
\end{tabular}
 \vspace{-0.4cm}
 \label{overhead}

%%%%add perf. eval
\end{table}


\subsection{Discussion}


To detect the faults in bitstream at run-time, we have implemented a hash-based authentication mechanism in CoRQ. However, fault detection might impact the functionality of the multi-tenant FPGA by restricting users from uploading their custom applications on the FPGA. Therefore, an on-chip fault-tolerant mechanism needs to be explored that detects and corrects errors on-the-fly. 

% In \cite{9643485}, the structure of the partial bitstream is divided into three segments. The first segment corresponds to the specific PRR of the FPGA where the bitstream will be configured. The second segment is configured with bits to shut down the selected PRR. The final segment corresponds to the design implemented by the bitstream e.g., a MAC, FFT etc. 

Using the fault localization scheme explained in Section VI.A, we can identify the specific blocks that are injected by faults. To mitigate the impact of faulty blocks, we can employ a fault-tolerant reconfiguration technique. We assume that we have the fault-free partial bitstreams hard-coded in the CoRQ memory. For a fault-injected bitstream $T$, let us denote the faulty block as $B_{flt}$, and the corresponding fault-free block as $B_{ff}$. As shown in \cite{9643485}, when a RO-based fault attack is detected, the specific PRR where the bitstream needs to be configured is disabled. We can employ the technique used in \cite{9643485} to 1) first disable the PRR where the bitstream needs to be configured, (2) replace $B_{flt}$ with $B_{ff}$, and (3) dynamically reconfigure the FPGA to bypass $B_{flt}$ and replace it with $B_{ff}$. This ensures that an user design is configured on the FPGA irrespective of faults injected into the original bitstream. We will explore this direction in future work.





==> Demo_FA.tex <==
\section{Experiments to calibrate the fault-injection mechanism}
\begin{figure}
\centering
\includegraphics[width=0.44\textwidth]{Figures/ro_fa.pdf}

\caption{Floorplan of the fault attack setup on the Pynq FPGA.}
\label{impl}
\vspace{-0.5cm}
\end{figure}
\begin{figure*}
\centering
\includegraphics[width=0.85\linewidth]{Figures/final_setup.pdf}
\caption{Hardware demonstration of RO-based fault attack on AES module implemented on the Pynq-Z1 FPGA (demo available in \cite{demo}): (a) An UART is used to establish the communication between the workstation and the FPGA; (b) UART RX transmits random plaintext input to the AES module; (c) Through UART TX, the AES-computed ciphertext is sent back from the FPGA to the workstation; (d) FPGA is programmed with the AES victim module and the attacker RO grid in a multi-tenant setup; (e) The blinking of the LED signal indicates an error in the computed ciphertext, indicating a fault attack; (f) Activation of this signal indicates that persistent fault injection is enabled during AES encryption.}
\label{setup}
\vspace{-0.4cm}

\end{figure*}

\begin{figure*}[!b]

\includegraphics[width=\linewidth]{Figures/merged.pdf}

\caption{Percentage of successful fault attacks versus range of toggling frequencies: ROs implemented with LUT utilization of (a) 15\% and (b) 30\%; self-clocked ROs implemented with LUT utilization of (c) 15\% and (d) 30\%.}
\label{attack}
\vspace{-0.5cm}
\end{figure*}

In this section, we outline the methodology for finding optimal fault-injection parameters of power-wasters to effectively induce fault attacks in partial bitstreams that are configured on the same FPGA. We demonstrate this through a fault attack experiment on an AES implementation operating on a Pynq-Z1 FPGA. The following subsections detail the experimental setup and describe the procedure for determining the appropriate fault-injection parameters.

\subsection{Ring Oscillator Circuits for Fault Injection}
% As a proof-of-concept to demonstrate successful fault injection using  RO circuits,  we perform a fault attack on an AES implementation running on the FPGA.

We develop a calibration algorithm to determine the fault-injection parameters such as duty cycle, toggling frequency, and number of RO instances that are sufficient to cause fault attacks on an AES module and generate faulty ciphertexts as output. An RO circuit consists of a chain of an odd number of inverters. The RO toggling frequency is given by $f_{toggle}=\frac{1}{2*n*t_d}$, where $n$ is the number of inverters in the RO circuit, and $t_d$ is the signal propagation delay. By tuning ROs to toggle on/off at resonant frequencies, they can cause significant voltage drops across the PDN of the FPGA. 
% Therefore, ROs are capable of inducing abrupt voltage fluctuations leading to fault injection \cite{gnad2020remote} in nearby modules not directly involved in the RO configuration.
\vspace{-0.1cm}







\subsection{Experimental Setup}
\vspace{-0.1cm}
Our experimental setup runs on a Xilinx Zynq XC7Z020 (Pynq-Z1) FPGA board with 53,200 LUT elements. The RO circuits used for generating voltage fluctuations are placed on the FPGA such that they occupy the majority of the FPGA LUTs. As mentioned in\cite{zhao2018fpga}, 16,000 ROs are sufficient to cause voltage drop-based fault attacks on a Zynq XC7Z020 FPGA. We keep the upper bound of RO instances as 50,000 to be consistent with experimental setups in prior work \cite{gnad2020remote}.

In a multi-tenant setup, AES is the victim module, and the RO grid is the attacker module. We develop a calibration algorithm (implemented in Python) that determines the desired configuration to activate the RO grid for a successful fault injection attack. Using this algorithm, we provide software commands from the workstation to the FPGA for dynamically sweeping the RO toggling frequency and the number of active ROs. We use UART to establish a communication between the FPGA and the workstation. We use the UART RX to transmit a plaintext input to the AES module implemented on the FPGA, and the UART TX to receive the ciphertext generated by AES. 

The calibration algorithm performs the following functions.

\begin{itemize}

    \item The parameters such as the RO toggling frequency, the duty cycle of RO activation, and the number of activated ROs at any given time are provided as a sequence of inputs to the FPGA via the UART.
    \item Subsequently, a random input plaintext is sent to the victim AES module implemented on the FPGA.
    \item Upon receiving the computed ciphertext from the AES module of the FPGA via UART, the result is compared with the golden ciphertext. If the computed ciphertext does not match the golden ciphertext, it indicates an error in the encryption process of the AES. 
\end{itemize}

% Once the fault-injection parameters are obtained, they remain fixed for the persistent reconfiguration fault attack on partial bitstreams uploaded via a reconfiguration manager.

% The default frequency of the clock source available on Pynq FPGA is 125 MHz. The clock frequency needed for running the UART and the AES module is 60 MHz. To adapt to a lower frequency, we use the Clocking Wizard available in the Vivado Design Suite to generate the required output clock frequency of 60 MHz. After configuring the Clocking Wizard, we generate the output products and integrate the new clock source into our FPGA design. We connect the 60 MHz output clock from the Clocking Wizard to the clock inputs of the UART and AES modules. 



% In Vivado, we update the .xdc (Xilinx Design Constraints) file to define the physical pins on the FPGA that are connected to the UART RX and TX ports. The updated .xdc file includes the following constraints:
% \begin{itemize}
%     \item \textit{set\_property} -dict { PACKAGE\_PIN \textit{Y19}   IOSTANDARD LVCMOS33 } [get\_ports { \textit{uart\_rxin} }]
%      \item \textit{set\_property} -dict { PACKAGE\_PIN \textit{Y17}   IOSTANDARD LVCMOS33 } [get\_ports { \textit{uart\_txout} }]
% \end{itemize}

The AES and RO circuits are written in VHDL and synthesized and implemented on Xilinx Vivado 2020.2. The floorplan of the experimental setup is shown in Fig. \ref{impl}. By default, the Vivado synthesis tool optimizes the ROs. To ensure that the ROs are not removed during synthesis, we apply the 'DON'T TOUCH' attribute to the RO instances in the HDL. 


\subsection{Selection of Fault-Injection Parameters}

We next perform run-time fault attack on AES using power-wasters to decide the optimal fault-injection parameters. In Fig. \ref{setup}, we demonstrate the hardware setup for a fault attack on the AES. The fault-injection parameters that are fed as inputs to the FPGA to activate the RO grid are as follows: [\textit{ro\_ena}, \textit{ro\_mask}, $f_{toggle}$, \textit{ro\_act}, $P$]. To initiate the fault-injection process in the AES, we activate the \textit{ro\_ena} signal. The \textit{ro\_mask} parameter enables a specific number of ROs at a time, \textit{ro\_act} is the duty cycle of the toggling RO, and $P$ is the input plaintext to the AES. 

We sweep the RO toggling frequency $f_{toggle}$ from 1 Hz to 1 MHz. For this experiment, the ROs are turned on and off at the toggling frequency. We show the percentage of fault injection attacks that occur at a range of $f_{toggle}$. The fault attack success rate is formulated as: $F_s=\frac{N_c}{N_t}\times 100\%$, where $N_t$ is the total number of attempts, i.e., the total number of different $f_{toggle}$ values that we use for toggling the ROs, and $N_c$ is the number of successful attempts (corresponding to specific values of $f_{toggle}$) at obtaining a faulty ciphertext. We report the number of obtained faulty ciphertexts out of $N_t = 10^4$ attempts. In scenarios where ROs utilize different percentages of the FPGA LUTs, partial bitstreams are generated separately for each case. These bitstreams are then individually reconfigured onto the FPGA. With 16,000 ROs, we obtain around 30\% utilization of FPGA LUTs. At 30\% LUT usage, we obtain $F_s$ = 35.91\%. We further reduce the LUT usage for ROs by masking specific bytes of \textit{ro\_mask}. For example, to enable 15\% of LUT usage implementing ROs, we set \textit{ro\_mask} as `cc'. At 15\% LUT usage, we obtain  $F_s$ = 34.68\%. For the frequency range ($f_l, f_u$), the percentage of successful fault attacks within this range is given by $F_t = \frac{N_{f_l- f_u}}{N_c}\times 100\%$, where $f_l$ and $f_u$ are the lower and upper frequency ranges, respectively. In Fig. \ref{attack}(a)-(b), we show the $F_t$ values when the ROs are increased from 15\% to 30\% LUT usage. A demo of the fault attack on AES with 30\% LUT utilization of ROs is shown in \cite{demo}.

We also show the severity of fault attack using a non-combinational RO, specifically the self-clocked RO. We observe that the self-clocked RO has fault-attack success rates of 35.74\% and 38.5\% for 15\% and 30\% LUT utilization, respectively. The high fault attack probabilities associated with these ROs indicate their effectiveness in causing fault attacks, while evading detection by AWS DRC. Fig. \ref{attack}(c)-(d) shows the $F_t$ values for different LUT utilization of ROs.

% \begin{figure}

% \includegraphics[width=\linewidth]{Figures/merged_sc.pdf}

% \caption{Percentage of successful fault attacks vs. range of toggling frequencies of self-clocked ROs. (a) 15\% of LUT usage of ROs, (b) 30\% of LUT usage of ROs.}
% \label{attack_sc}
% \vspace{-0.4cm}
% \end{figure}

These preliminary results help us obtain the appropriate fault-injection parameters of the RO grid for enabling a fault attack on a victim AES module in a multi-tenant setup. Subsequently, we keep these parameters fixed while evaluating the impact of a persistent reconfiguration fault attack on several partial bitstreams that are configured to the FPGA via a reconfiguration manager. 




==> Discussion.tex <==
\section{Discussion}

To detect the faults in bitstream at run-time, we have implemented an ASCON hash-based authentication mechanism in the CoRQ. However, fault detection might impact multi-tenancy by restricting users from uploading their modules on the FPGA. This impacts the functionality of the multi-tenant FPGA as it is expected to cater to the needs of multiple users to upload their specific applications on the FPGA. Therefore, an on-chip fault-tolerant mechanism needs to be explored that detects and corrects errors on-the-fly. 

% In \cite{9643485}, the structure of the partial bitstream is divided into three segments. The first segment corresponds to the specific PRR of the FPGA where the bitstream will be configured. The second segment is configured with bits to shut down the selected PRR. The final segment corresponds to the design implemented by the bitstream e.g., a MAC, FFT etc. 
Using the fault localization scheme explained in Section VI, we can identify the specific blocks that are injected by faults. To mitigate the impact of faulty blocks, we can employ a fault-tolerant reconfiguration technique. We assume that we have the fault-free partial bitstreams hard-coded in the CoRQ memory. For a fault-injected bitstream $T$, let us denote the faulty block as $B_{flt}$, and the corresponding fault-free block as $B_{ff}$. As shown in \cite{9643485}, when a RO-based fault attack is detected, the specific PRR where the bitstream needs to be configured is disabled. We can employ the technique used in \cite{9643485} to 1) first disable the PRR where the bitstream needs to be configured, (2) replace $B_{flt}$ with $B_{ff}$, and (3) dynamically reconfigure the FPGA to bypass $B_{flt}$ and replace it with $B_{ff}$. This ensures that an user design is configured on the FPGA irrespective of faults injected into the original bitstream. We will explore this direction in future work.


\vspace{-0.1cm}

==> Experiments_to_do.tex <==
Brief Idea: Causing faults while partial reconfiguration in an FPGA
happens. The main threat model is an attacker that wants to manipulate
bitstreams of other tenants in a Multi-Tenant FPGA. The attacker would
be able to manipulate part of the bitstream that is getting written into
the confguration memory. A new suggestion was, that the attacker might
even manipulate the System/Supervisor region (if also in reconfigurable
logic). Partial reconfiguration bitstreams contain a "region select", so
it is feasible. I.e. any time reconfiguration happens, any part of the
FPGA could be permanently changed by an attacker.

Required: Ability to permanently affect the bitstream of a
co-tenant by attacking it while partially reconfiguring.

    * Required: Explain how CoRQ with CRC is not a full countermeasure.
Then we can integrate a proper checksum (e.g. SHA2/3) into CoRQ as a
secure countermeasure. Hassan said that this is rather easily possible.
We might still need to discuss details here.

    * Optional: Ability to affect a supervisor or other random region by
affecting the region selection specifically.

    * Future work: Try to affect even more specific bits/bytes either in
the region selection or elsewhere in the bitstream. I think this might
be relatively hard to do and needs a lot of time for doing many
experiments, so almost impossible in 2 months. It is better to explore
later.
 

==> JC_to_add.tex <==
### Input from Hassan ###
\subsection{Comparison to Runtime Fault Injection Attacks}

Several previous works discussed fault injection at runtime.
Ref.~\cite{krautter2018fpgahammer} used ISCAS-based circuits to inject faults on AES.
Refs.~\cite{duplicated_entry_9643485,gnad2020remote} explored the right combinations for injecting faults on specific types of FPGAs.
Ref.~\cite{boutros20} targets injecting faults to DNNs.
All these works require that the attack to be running during the whole runtime of the victim accelerator to be effective. 
If the victim accelerator runs for two hours, the attack will have to run for two hours.
This put the attack at risk as simple monitoring of the power activity can give it away.
In contrast, our attack causes persistent faults.
It has to run only during the upload of the bitstream which is usually in the range of milliseconds.
Once, the upload is done, the attack can stop and the uploaded bitstream will already have the faults in it.
Therefore, even if our attack is detected at one point, it will already have affected the accelerator and the fault will persist even if the attack is stopped.




The voltage drop across the PDN is formulated as: $V_{drop}=IR + L\frac{di}{dt}$. 



The attacks are timed to inject faults into a bitstream \textbf{while} it is being reconfigured on the RM, and cease once the bitstream is fully loaded onto the RM. As highlighted in \cite{10.1145/3451236}, voltage sensors typically take a longer time to detect most attacks. The proposed attack is designed to be active only during the reconfiguration process, which lasts only milliseconds. Due to this brief duration, it avoids detection. It is important to note that the fault introduced during the bitstream reconfiguration is not just transient; the injected fault becomes embedded within the bitstream itself.
